SLOT: Structuring the Output of Large Language Models

Structured outputs are essential for large language models (LLMs) in critical applications like agents and information extraction. Despite their capabilities, LLMs often generate outputs that deviate from predefined schemas, significantly hampering reliable application development. We present SLOT (Structured LLM Output Transformer), a model-agnostic approach that transforms unstructured LLM outputs into precise structured formats. While existing solutions predominantly rely on constrained decoding techniques or are tightly coupled with specific models, SLOT employs a fine-tuned lightweight language model as a post-processing layer, achieving flexibility across various LLMs and schema specifications. We introduce a systematic pipeline for data curation and synthesis alongside a formal evaluation methodology that quantifies both schema accuracy and content fidelity. Our results demonstrate that fine-tuned Mistral-7B model with constrained decoding achieves near perfect schema accuracy (99.5%) and content similarity (94.0%), outperforming Claude-3.5-Sonnet by substantial margins (+25 and +20 percentage points, respectively). Notably, even compact models like Llama-3.2-1B can match or exceed the structured output capabilities of much larger proprietary models when equipped with SLOT, enabling reliable structured generation in resource-constrained environments.

==> tables/tpot.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{ p{4cm}|p{2cm}||c|c|c|c|c||c }
        \hline
       \multirow{2}{4cm}{Base LLM (host + \newline structured output support)}&\multirow{2}{4cm}{FT dataset}&\multicolumn{6}{c}{TPOT (ms)} \\
       \cline{3-8}
       && WebNLG&E2E NLG&WikiBio&ToTTo&GitHub&Avg\\
       \hline
       \hline
       \multirow{2}{4cm}{Llama 3.2 1B\newline(self-hosted)}&-&19.51&15.57&20.04&19.56&19.98&18.93\\
        \cline{2-8}
       &Pub + Synth&15.65&19.79&16.5&19.81&16.25&17.60\\
       \hline
       \multirow{2}{4cm}{Llama 3.2 1B\newline(self-hosted + Outlines)}&-&0.06&0.06&0.06&0.05&0.06&0.06\\
       \cline{2-8}
       &Pub+ Synth&0.05&0.06&0.06&0.05&0.05&0.05\\
       \hline
       \hline
       \multirow{2}{4cm}{Llama 3.2 3B\newline(self-hosted)}&-&25.66&26.37&27.58&26.02&34.64&28.05\\
        \cline{2-8}
       &Pub + Synth&27.41&33.74&28.92&26.32&27.09&28.70\\
       \hline
        \multirow{2}{4cm}{Llama 3.2 3B\newline(self-hosted + Outlines)}&-&0.05&0.03&0.05&0.06&0.05&0.05\\
       \cline{2-8}
       &Pub + Synth&0.06&1.33&0.05&0.06&0.05&0.31\\
       \hline
       \hline
       \multirow{2}{4cm}{Mistral 7B (v0.2)\newline(self-hosted)}&-&30.79&37.25&37.87&37.17&35.91&35.80\\
       \cline{2-8}
       &Pub+ Synth&32.97&32.51&40.21&39.22&36.43&36.27\\
       \hline
       \multirow{2}{4cm}{Mistral 7B (v0.2)\newline(self-hosted + Outlines)}&-&0.05&0.05&0.06&0.06&0.05&0.05\\
       \cline{2-8}
       &Pub+ Synth&0.07&0.07&0.07&0.05&0.05&0.06\\
       \hline
       \hline
    \end{tabular}
    \caption{Time-Per-Output-Token (TPOT) of different base and fine-tuned LLMs}
    \label{tab:content_sim}
\end{table*}
